On the Feasibility of Machine Learning Augmented Magnetic Resonance for Point-of-Care Identification of Disease

Early detection of many life-threatening diseases (e.g., prostate and breast cancer) within at-risk population can improve clinical outcomes and reduce cost of care. While numerous disease-specific "screening" tests that are closer to Point-of-Care (POC) are in use for this task, their low specificity results in unnecessary biopsies, leading to avoidable patient trauma and wasteful healthcare spending. On the other hand, despite the high accuracy of Magnetic Resonance (MR) imaging in disease diagnosis, it is not used as a POC disease identification tool because of poor accessibility. The root cause of poor accessibility of MR stems from the requirement to reconstruct high-fidelity images, as it necessitates a lengthy and complex process of acquiring large quantities of high-quality k-space measurements. In this study we explore the feasibility of an ML-augmented MR pipeline that directly infers the disease sidestepping the image reconstruction process. We hypothesise that the disease classification task can be solved using a very small tailored subset of k-space data, compared to image reconstruction. Towards that end, we propose a method that performs two tasks: 1) identifies a subset of the k-space that maximizes disease identification accuracy, and 2) infers the disease directly using the identified k-space subset, bypassing the image reconstruction step. We validate our hypothesis by measuring the performance of the proposed system across multiple diseases and anatomies. We show that comparable performance to image-based classifiers, trained on images reconstructed with full k-space data, can be achieved using small quantities of data: 8% of the data for detecting multiple abnormalities in prostate and brain scans, and 5% of the data for knee abnormalities. To better understand the proposed approach and instigate future research, we provide an extensive analysis and release code.

==> sections/empirical.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.5\textwidth]{figures/results/task_diff.pdf}
\caption{\textbf{Exploring the limits of under-sampling for classification}. Shows the performance of \textsc{emrt} for  
classification, using sampling rates $\alpha \in \{$5$\%, $8$\%, $10$\%, $12.5$\%, 100\%\}$. 
As you can observe the difference performance deterioration is not significant, and at lower sampling rates, the \textsc{auroc} is comparable to the fully-sampled \textsc{k}-space classifier.}\label{fig:empirical_1}
\end{figure}



To better understand the working of \textsc{arms}
we analyze its different components. 
Recall the three key characteristics of \textsc{arms}:
(1) it works directly with the complex valued $k$-space data,
(2) the classifier $q_{\text{val}}$ is trained using random
subsets of the $k$-space data, and
(3) it learns the under-sampling pattern over
the $k$-space data matrix.
To understand the role of these characteristics 
we disentangle their contributions.
We achieve this by asking the following questions:
{\bf Q1.} Do we need high-resolution images to accurately 
identify diseases? 
{\bf Q2.} Is there any benefit in classifying directly 
from the \textit{k}-space data?
{\bf Q3.} What role does the random subset training
of classifier $q_{\text{val}}$ play
in its performance?
{\bf Q4.} What role does the learned under-sampling 
pattern play in \textsc{arms}'  performance?



\textbf{What role does the random subset training
of the \textsc{arms} classifier $q_{\text{val}}$ play
in its performance?}
We examine whether training a direct $k$-space classifier with
random under-sampling patterns has any benefit compared to
training a classifier with a fixed under-sampling pattern.
To that end, we compare the performance of the
\textsc{arms} classifier $q_{\text{val}}$ to a model
trained with the fixed but learnt under-sampling pattern.
We use the under-sampling pattern learnt by \textsc{arms}
as the input to this classifier.
The architecture of the two classifiers were identical.
In \Cref{fig:empirical_1}, we observe that for most
sampling rates the classifier trained with random
under-sampling patterns outperforms the
classifier trained with a single fixed but learnt
under-sampling pattern.
Training using the random under-sampling
patterns act as a regularizer which leads to
better generalization performance.


\input{figures/results/empirical_1}

\input{figures/results/kspace_vs_image}

\input{figures/results/fixed_v_center}


